Cost Optimized Scheduling in Modular Electrolysis Plants

In response to the global shift towards renewable energy resources, the production of green hydrogen through electrolysis is emerging as a promising solution. Modular electrolysis plants, designed for flexibility and scalability, offer a dynamic response to the increasing demand for hydrogen while accommodating the fluctuations inherent in renewable energy sources. However, optimizing their operation is challenging, especially when a large number of electrolysis modules needs to be coordinated, each with potentially different characteristics. To address these challenges, this paper presents a decentralized scheduling model to optimize the operation of modular electrolysis plants using the Alternating Direction Method of Multipliers. The model aims to balance hydrogen production with fluctuating demand, to minimize the marginal Levelized Cost of Hydrogen (mLCOH), and to ensure adaptability to operational disturbances. A case study validates the accuracy of the model in calculating mLCOH values under nominal load conditions and demonstrates its responsiveness to dynamic changes, such as electrolyzer module malfunctions and scale-up scenarios.

==> 999_State_of_the_Art_old.tex <==
\section{State of the Art}\label{sec:stateoftheart}
\subsection{Technical Background}
Water electrolysis is a key technology for producing green hydrogen from renewable energy sources. The literature extensively covers various types of water electrolysis [Quellen], including \textit{Alkaline Electrolysis} (AEL), \textit{Proton Exchange Membrane Electrolysis} (PEMEL), \textit{High-Temperature Electrolysis} (HTEL), and \textit{Anion Exchange Membrane Electrolysis} (AEMEL). These electrolysis technologies are currently employed in the market, each offering distinct characteristics, limitations and applications for hydrogen production \cite{LKL+23}.

Assessing the economic feasibility and efficiency of hydrogen production from these diverse electrolysis technologies is essential in driving forward the adoption of green hydrogen. One widely used metric for this purpose is the \textit{Levelized Cost of Hydrogen} (LCOH), which provides a standardized evaluation basis for comparing the cost-effectiveness of hydrogen production across different electrolysis technologies and plant configurations (Bessere Quelle) \cite{MAH23}. LCOH takes into account various factors such as capital expenditures (CapEx), operational expenditures (OpEx), operation \& maintenance (O\&M) and efficiency, offering valuable insights into the overall cost structure of green hydrogen production \cite{GVE+22, BRP22}. 

%LCOH-Figure
\begin{figure}[h]
    \centering
    \resizebox{.99\linewidth}{!}{\input{Figures/LCOH}}
    \caption{Breakdown of OpEx and CapEx contributions to mLCOH for a 10MW PEM electrolyzer at varying power levels with an electricity cost of 0.04 €/kWh (Illustration adapted from \cite{GVE+22})}
    \label{fig:LCOH}
\end{figure}

It is worth noting that while LCOH is primarily employed for the assessment and selection of electrolysis technologies \cite{MAH23, SPN+22}, some recent works, such as \cite{GVE+22, VCF+22}, have explored the potential of utilizing LCOH for operational optimization as well. 

In their study, \cite{BRP22} examines the correlation between the economics and cost factors of LCOH concerning operational aspects. The results reveal that electrolyzers with higher CapEx must be operated at higher load factors to achieve the lowest LCOH. Conversely, reducing CapEx shifts the minimum LCOH to lower utilization rates, as the cost of electrical energy becomes a larger proportion of the total cost. This highlights the significance of lower CapEx in providing greater operational flexibility, making electrolyzers more economically dynamic and adaptable in their operation.

In this regard, the concept of \textit{marginal LCOH} (mLCOH) has been introduced, as illustrated in \autoref{fig:LCOH}, where LCOH is calculated periodically (e.g. hourly) as a function of the power. mLCOH allows for a more detailed and frequent analysis, as it considers factors such as the current electricity price, enabling periodic adjustments in the operational optimization process. To the best of our knowledge, the application of mLCOH for load distribution optimization in modular, heterogeneous electrolysis plants remains a relatively unexplored area of research.

Nonetheless, due to the versatility and well-established nature of LCOH, including mLCOH, these metrics hold significant promise in effectively capturing the heterogeneity of electrolysis technologies and, consequently, optimizing load distribution in modular, heterogeneous electrolysis plants, as addressed in the first research question. The findings from \cite{BRP22}, which examine the correlation between economics and LCOH cost factors, further support their suitability for load distribution optimization. Understanding how CapEx and operational aspects influence LCOH enables informed decision-making and enhanced operational flexibility in heterogeneous electrolysis plants

Based on the existing work on modular electrolysis plants and their requirements \cite{HSM+23}+ETFAWIP, the following section outlines the specific requirements that the MAS should incorporate to effectively optimize load distribution: 

\begin{req}  
    \item \textbf{Predictive Planning of Operating States:} 
    The system must determine the operating state (e.g., idle, production or standby) of the electrolyzers. It must consider technical limitations (e.g., start-up time) to ensure they are operated optimally and in accordance with a variable hydrogen demand.
    
    \item \textbf{Decentralized Cost-Optimized Load Distribution:}
    The system must execute load distribution in a decentralized manner among heterogeneous electrolyzers to satisfy variable hydrogen demand while minimizing costs.

    \item \textbf{Adaption to Demand and Supply Fluctuations:}
    The system must adapt to short-term fluctuations in hydrogen demand and electrical supply. This entails dynamically adjusting the load distribution on among operational electrolyzers to ensure uninterrupted hydrogen production, even during periods of fluctuating demand or varying energy availability.

    \item \textbf{Resilience to Electrolyzer Failures:}
    The system must demonstrate robustness by responding to electrolyzer failures or malfunctions. In such scenarios, the system must initiate a load redistribution process to ensure uninterrupted hydrogen production. The load distribution among the operational electrolyzers that remain must be dynamically adjusted to compensate for the failed electrolyzer.

    \item \textbf{Efficient Operation considering Degradation:} The system should implement resource-efficient operation strategies to minimize frequent load changes and start-stop cycles, thereby mitigating potential electrolyzer degradation risks \cite{GVE+22, BRP22}. 
    
    \item \textbf{Electrolyzer Monitoring and Control:} The system must monitor the current state of electrolyzers and convert the optimized operational points, derived from the cost-optimized  load distribution, into actionable control commands. 
    
\end{req}

\subsection{Related Works}
Several studies have been conducted on the operational optimization of electrolysis plants. Additionally, there has been relevant research in the context of decentralized scheduling of energy applications, economic dispatch or agent-based scheduling. The following section presents works from both domains.

%Kaligh
In \citet{KGM+22}, a stochastic, agent-based model for the planning of a Multi-Vector Microgrid is presented, considering electricity, hydrogen, and gas energy sectors. The model aims to optimize cooperation and coordination between these energy sectors, taking into account uncertainties in energy generation, storage, and demand. Coupling constraints are described using the extended \textit{Lagrange-Relaxation} (ALR) and the \textit{Alternating Direction Method of Multipliers} (ADMM) to achieve consensus between agents and energy sectors. 
%The results of a case study demonstrate that the proposed model efficiently allocated the available energy, meeting all energy demands, and the ADMM method showed rapid convergence.

%Vincenti
In \citet{VCF+22}, the study optimizes the size and schedule of a Power-to-Hydrogen system linked to a hydrogen refueling station (HRS). The goal is to determine the optimal system size and schedule for hydrogen production considering different electricity supply scenarios (grid, solar and hydro). The results provide insights into design and operational parameters while considering minimal LCOH for refueling vehicles.

%Flamm
In \citet{FPB+21}, a real-time optimization approach for electrolyzer control is introduced. The model utilizes a \textit{Mixed-Integer Linear Programming} (MILP) formulation to capture the non-linear characteristics of a PEM electrolyzer. By optimizing every minute, the system meets hydrogen demand at a lower cost compared to linearized models. The optimization employs a control system hierarchy, with high-level MATLAB calculations determining the power value for the electrolyzer and transmitting commands to the medium and low-level controls.

%Varela
In \citet{VMZ21}, a scheduling model for alkaline water electrolysis is developed as a MILP with decision variables representing operational states and transitions. The model incorporates operational characteristics as constraints, considering three operational states (production, standby, idle) and transitions (cold/full start, shutdown) for an accurate representation of electrolysis operations. Continuous variables are used for power and hydrogen flows. The model enables optimal sizing of electrolyzers and provides production schedules based on extensive datasets of intermittent energy and power prices.

%Ginsberg
\citet{GVE+22} introduces a techno-economic model for dynamically optimizing PEM electrolyzer operation. The model enables the determination of an optimal current density while considering the impact of increased degradation rates. Through this approach, the study predicts and compares the LCOH for different operation methods and power densities, encompassing various cost factors such as CapEx, OpEx and O\&M costs.

%Dong Isolated Hydrogen Microgrid
In \citet{DSM+23}, a forecast-driven stochastic scheduling strategy is proposed for optimizing the operation of an isolated hydrogen microgrid. The study introduces an energy management system that utilizes forecast-driven stochastic optimization methods, including bidirectional and long short-term memory convolutional neural networks for forecasting changes in wind power and load over 24 hours. The system employs deep reinforcement learning for stochastic optimization scheduling to minimize the economic cost of the microgrid lifecycle.

%Li, Fei
In \citet{LFL+22}, a Multi-Unit control strategy for electrolyzers is explored, taking into account the start-stop times. The main objective is to develop a control strategy that optimizes the energy consumption by considering the start-stop times of the electrolyzers. 

%Jiang, Yuewen
In \citet{JLZ23}, a scheduling model for distributed HRSs is introduced, aiming to maximize the revenue of HRSs over one day. To handle multiple variables and complex nonlinear constraints, the paper develops a transfer multi-agent reinforcement learning algorithm. The approach treats different variables, like the input power of each HRS, as individual agents to achieve the joint optimal operation of multiple HRSs.

%Safari, Amin
In \citet{SANA22}, the paper addresses the stochastic day-ahead optimal scheduling of multimicrogrids with the objective of minimizing operational costs. To solve the optimization problem, the paper proposes the use of the ADMM to facilitate computation and reduce computational effort.

\begin{table}[ht]
  \centering
  \caption{Evaluation of scientific research. Semantics: \fulfill{100} fulfilled,\newline \fulfill{0} not fulfilled, \fulfill{50} partially fulfilled, [-] not evaluable}
  \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
    & \begin{sideways}\textbf{REQ1}\;\,\end{sideways} & \begin{sideways}\textbf{REQ2}\end{sideways} & \begin{sideways}\textbf{REQ3}\end{sideways} & \begin{sideways}\textbf{REQ4}\end{sideways} & \begin{sideways}\textbf{REQ5}\end{sideways} & \begin{sideways}\textbf{REQ6}\end{sideways}\\
    \hline
    \citet{KGM+22} & \fulfill{100} & \fulfill{0} & \fulfill{0} & X & \fulfill{100} & \fulfill{0}  \\
    \hline
    \citet{VCF+22} & \fulfill{100} & \fulfill{0} & \fulfill{0} & X & \fulfill{100} & \fulfill{0} \\
    \hline
    \citet{FPB+21} & \fulfill{0} & \fulfill{0} & \fulfill{0}  & X & \fulfill{100} & \fulfill{100} \\
    \hline
    \citet{VMZ21} & \fulfill{100} & \fulfill{50} & \fulfill{0}  & X &  \fulfill{0} & \fulfill{0}  \\
    \hline
    \citet{GVE+22} & \fulfill{0} & \fulfill{0} & [-] & X &  \fulfill{100} & \fulfill{0} \\
    \hline
    \citet{DSM+23} & \fulfill{0} & [-] & [-] & X & \fulfill{100} & \fulfill{0}  \\
    \hline
    \citet{LFL+22} & \fulfill{100} & \fulfill{50} & \fulfill{0}  & X & \fulfill{100} & \fulfill{0}  \\
    \hline
    \citet{JLZ23} & \fulfill{100} & \fulfill{50} & [-] & X &  \fulfill{0} & \fulfill{0}  \\
    \hline
    \citet{SANA22} & \fulfill{0} & [-] & [-] & X & \fulfill{0} & \fulfill{0}  \\
    \hline
  \end{tabular}
  \label{tab:requirementsRelatedWorks}
\end{table}


Existing research focuses on optimizing homogeneous electrolysis plants concerning either electrolyzer technology or electrolyzer capacity. While some earlier studies like \cite{VCF+22} and \cite{VMZ21} touch on CaPex, a more detailed analysis, considering CapEx per electrolysis PEA, is essential for effective load distribution in modular electrolysis plants. Moreover, it's worth noting that very few works delve into the practical translation of optimization results into actionable control, monitoring, and command implementation at the field level; most tend to concentrate solely on optimization aspects. This manifests itself in the fact that potential failures or disruptions cannot be adequately taken into account.

The work presented in \cite{SANA22} underscores the benefits of decentralized approaches in terms of system scalability, achieved without requiring substantial alterations to the central control. This approach, which has proven effective across various application scenarios \cite{KGM+22, JLZ23}, utilizes methodologies such as agents and ADMM. 
%Importantly, the characteristics inherent to modular, heterogeneous electrolysis plants—such as distributed intelligence, expandability, and adaptability—align well with this approach, making it potentially applicable and beneficial.






==> 99_Notes.tex <==

\textbf{Warum Agenten?}
\begin{itemize}
    \item Modulare Anlagen kapseln Services $\rightarrow$ Agenten kapseln Zustände, Ziele und Pläne $\rightarrow$ Modulare Elektrolyseanlagen
    \item Strukturell veränderbare Systeme $\rightarrow$ Struktur ändert sich dynamisch (modulare Anlagen, Wandelbarkeit)
    \item Kooperative Systeme
    \item aus Artans Paper zu Herausforderungen: Modular electrolysis plants in particular offer the possibility of reacting flexibly to renewable power generation and increasing demand [Lange et al. 2023]. This results in an increase in physical flexibility of electrolysis plants. Electrolysis modules can be added, removed or replaced by larger/smaller ones. However, this must also be accompanied by a higher flexibility of the plant’s automation [Lange et al. 2023, Bittorfet al. 2022].
    \item aus Artans Paper: Furthermore a suitable decentralized and agent-based control system is designed to support flexible operation of modular electrolysis plants [QUELLEN].
    \item In 10.1109/ICAdLT.2014.6866316       wird zusammengefasst, dass sich MAS für das Scheduling unter unsicheren Bedingungen eignen (als reaktiver Ansatz)
\end{itemize}

\textbf{Warum ADMM?}
\begin{itemize}
    \item In \citet{SFZ+21} wird dargestellt, dass ADMM deutlich schneller ist, als ein zentraler Algorithmus, allerdings nur geringfügig schlechtere Optimierungsergebnisse aufweist. 
\end{itemize}

Zu den related Works:

Es zeigt sich, dass
- im Kontext der Betriebsoptimierung nur homogene Elektrolyseanlagen betrachtet werden,
- In einigen bestehenden Arbeiten werden zwar teilweise Investitionskosten betrachtet (\cite{YPC+22, VMZ21}) allerdings reicht diese grobe Betrachtung nicht aus und muss pro Elektrolyse-Modul herangezogen werden, um ein geeignetes Scheduling in modularen, heterogenen Elektrolyseanlagen durchführen zu können
- In \cite{SANA22} wird beschrieben, dass es in dezentralisierten Method einfacher ist das System auszuweiten, ohne spezifische Anforderungen an einem centralen Controller durchzuführen (Moreover, it is easier in decentralised methods to expand the system without any specific changes in the central controller). + da sich Agenten, ADMM, verteilte Optimierung im Bereich von Mikrogrids als sehr probates Instrument erwiesen haben. Das Problem durchaus übertragbar ist auf den Anwendungsfall modularer, heterogener Elektrolysenanlagen, allerdings noch auf die spezifischen Anforderungen zugeschnitten werden muss.

\begin{itemize}
    \item \textit{Related Works beschreiben (Agenten und Betriebsoptimierung) , Tabelle: Abgleich der Anforderungen aus Technical Background}
    \item $\rightarrow$ Heterogenität noch nicht gelöst, daher neue Grundlage. Flexibilität und Wandelbarkeit auch nicht.
    \item als Ergebnis soll rauskommen, da sich Agenten, ADMM, verteilte Optimierung im Bereich von Mikrogrids als sehr probates Instrument erwiesen haben. Das Problem durchaus übertragbar ist auf den Anwendungsfall modularer, heterogener Elektrolysenanlagen, allerdings noch auf die spezifischen Anforderungen zugeschnitten werden muss. 
    \item Zudem kann gezeigt werden, dass bisher nur homogene Anlagen im Kontext der Betriebsoptimierung von Elektrolyseanlagen betrachtet wurden. Um verschiedene Kosten (CapEx, OpEx, Effizienz) in Relation zu setzen kann aus Ginnsberg die LCOH als standardisierte Bewertungsgrundlage herangezogen werden.
    \item In einigen bestehenden Arbeiten werden zwar teilweise Investitionskosten betrachtet (s. \cite{YPC+22, VMZ21}) allerdings reicht diese grobe Betrachtung nicht aus und muss pro Elektrolyse-Modul herangezogen werden, um ein geeignetes Scheduling durchführen zu können
    \item In \cite{SANA22} wird beschrieben, dass es in dezentralisierten Method einfacher ist das System auszuweiten, ohne spezifische Anforderungen an einem centralen Controller durchzuführen (Moreover, it is easier in decentralised methods to expand the system without any specific changes in the central controller).  
\end{itemize}
